Learning to Play Guess Who? and Inventing a Grounded Language as a Consequence

Acquiring your first language is an incredible feat and not easily duplicated. Learning to communicate using nothing but a few pictureless books, a corpus, would likely be impossible even for humans. Nevertheless, this is the dominating approach in most natural language processing today. As an alternative, we propose the use of situated interactions between agents as a driving force for communication, and the framework of Deep Recurrent Q-Networks for evolving a shared language grounded in the provided environment. We task the agents with interactive image search in the form of the game Guess Who?. The images from the game provide a non trivial environment for the agents to discuss and a natural grounding for the concepts they decide to encode in their communication. Our experiments show that the agents learn not only to encode physical concepts in their words, i.e. grounding, but also that the agents learn to hold a multi-step dialogue remembering the state of the dialogue from step to step.

==> GuessWhomodel.tex <==
        \def\layersep{5}
    \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep cm,        invisibleboxnode/.style={rounded corners=3pt, draw=none, fill=none, very thick, minimum width=50mm, minimum height=10mm, align=center},
]
        \tikzstyle{every pin edge}=[<-,shorten <=1pt]
        \tikzstyle{rnn}=[rectangle,minimum width=1.5cm,minimum height=0.75cm, fill=blue!15, draw=blue!50, thick,inner sep=1pt]{}
        \tikzstyle{elemwise}=[rectangle,minimum width=3cm,minimum height=0.75cm, fill=green!15, draw=green!50, thick,inner sep=1pt]{}
        \tikzstyle{qvals}=[rectangle,minimum width=3cm,minimum height=0.75cm, fill=red!15, draw=red!50, thick,inner sep=1pt]{}
        \tikzstyle{variables}=[rectangle,minimum width=3cm,minimum height=0.75cm, thick,inner sep=1pt]{}        
        
            % \node[rnn, pin=left:$s_{0}$] (R1-1) at (\layersep cm, 0 cm) {};


            % \node[rnn,pin=left:$s_{1,0}$] (R2-1) at (\layersep cm, -\layersep*0.5 cm) {};
            
            % \node[rnn, pin={[pin edge={->}]right:$s_{3}$   ...}] (R1-3) at (\layersep*3 cm, 0 cm) {};
            % \node[rnn, pin={[pin edge={->}]right:$s_{1,3}$   ...}] (R2-3) at (\layersep*3 cm, -\layersep*0.5 cm) {};
        
        \foreach \name / \y in {1,...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[elemwise, pin=below:{\includegraphics[width=.05\textwidth]{guess_who/7.png}}
            {\includegraphics[width=.05\textwidth]{guess_who/22.png}}
            {\includegraphics[width=.05\textwidth]{guess_who/8.png}}
            {\includegraphics[width=.05\textwidth]{guess_who/5.png}}] (E1-\name) at (\layersep*\y cm, -\layersep*1*0.3 cm) {Elemwise add};
        
        \foreach \name / \y in {1,...,2}
            \node[qvals] (Q1-\name) at (\layersep*\y cm, \layersep*0.3 cm) {DRU};
            
        \foreach \name / \y in {3,...,3}
            \node[qvals] (Q1-\name) at (\layersep*\y cm, \layersep*0.3 cm) {$\epsilon$-greedy};
            
        \foreach \name / \y in {1,...,2}
            \node[variables] (V1-\name) at (\layersep*\y cm, \layersep*0.3 cm + 0.25*\layersep cm) {$\hat{m}_{\y}^1$};
            
        \foreach \name / \y in {3,...,3}
            \node[variables] (V1-\name) at (\layersep*\y cm, \layersep*0.3 cm + 0.25*\layersep cm) {$u^1$, \text{reward}};
  

        \foreach \name / \y in {1,...,3}
            \node[rnn] (R1-\name) at (\layersep*\y cm, 0 cm) {GRU};
            
        % \foreach \name / \y in {1,...,3}
        %     \node[rnn] (R2-\name) at (\layersep*\y cm, -\layersep*0.5 cm) {GRU};
            
        % \foreach \name / \y in {2, ...,3}
        %     \pgfmathsetmacro{\source}{int(\name-1)}
        %     \path (R2-\source) edge node[above, midway] {$h_{1,\source}$} (R2-\name);

        \foreach \name / \y in {2, ...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (R1-\source) edge node[above, midway] {$h^1_{\source}$} (R1-\name);


        % \foreach \name / \y in {1, ...,3}
        %     \path (R2-\name) edge node[right, midway] {$h_{1,\y}$} (R1-\name);
        
        \foreach \name / \y in {1, ...,2}
            \path (R1-\name) edge node[right, midway] {${m_\y^1}$} (Q1-\name);
            
        \foreach \name / \y in {3, ...,3}
            \path (R1-\name) edge node[right, midway] {${Q^1}$} (Q1-\name);
            
        \foreach \name / \y in {1, ...,3}
            \path (E1-\name) edge node[right, midway] {$z_{\y}^1$} (R1-\name); 
            
        \foreach \name / \y in {1, ...,3}
            \path (Q1-\name) edge (V1-\name);    
         
        \def\separate{1.3}
  
            
        %%%%%
        
        % \node[rnn, pin=left:$s_{0}$] (R21-1) at (\layersep cm + 0.5*\layersep cm,                    \separate*\layersep cm) {};
        
          \foreach \name / \y in {1,...,2}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[elemwise, pin=above:{\includegraphics[width=.05\textwidth]{guess_who/5.png}}] (E21-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm +\layersep*0.3 cm) {Elemwise add};
        
        \foreach \name / \y in {1,...,2}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[qvals] (Q21-\name) at (\layersep*\y cm +  0.5*\layersep cm, \separate*\layersep cm -\layersep*0.3 cm) {DRU};
            
         \foreach \name / \y in {1,...,2}           
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[variables] (V21-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm - \layersep*0.3 cm - 0.25*\layersep cm) {${\hat{m}_{\y}^2}$(yes/no)};
            
        \foreach \name / \y in {1,...,2}
            \node[rnn] (R21-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm) {GRU};
            
        % \foreach \name / \y in {1,...,2}
        %     \node[rnn] (R22-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm +\layersep*0.5 cm) {GRU};
            
        % \foreach \name / \y in {2, ...,2}
        %     \pgfmathsetmacro{\source}{int(\name-1)}
        %     \path (R22-\source) edge node[above, midway] {$h_{1,\source}$} (R22-\name);

        \foreach \name / \y in {2, ...,2}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (R21-\source) edge node[above, midway] {$h^2_{\source}$} (R21-\name);


        % \foreach \name / \y in {1, ...,2}
        %     \path (R22-\name) edge node[right, midway] {$h_{1,\y}$} (R21-\name);
        
        \foreach \name / \y in {1, ...,2}
            \path (R21-\name) edge node[right, midway] {${m_t^2}$} (Q21-\name);
            
        \foreach \name / \y in {1, ...,2}
            \path (E21-\name) edge node[right, midway] {$z_{\y}^2$} (R21-\name); 
        
        \foreach \name / \y in {1, ...,2}
            \path (Q21-\name) edge (V21-\name);
            
        \foreach \name / \y in {2, ...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (V21-\source) edge[thick,draw=black!85]  (E1-\name.160);
        \foreach \name / \y in {1, ...,2}
            \path (V1-\name) edge[thick,draw=black!85] (E21-\name.200);
            
         \node[draw,dotted,very thick,draw=black!60,fit=(R21-1) (R21-2) (Q21-1) (Q21-2) (E21-1) (E21-2)] (a2) {};
        
        \node[draw,dotted,very thick,draw=black!60,fit=(R1-1) (R1-3) (Q1-1) (Q1-3) (E1-1) (E1-3)] (a1) {};
         
        \node[invisibleboxnode,rotate=90]  (answering agent)  at (1*\layersep cm, \separate*\layersep cm) {answering agent};
        
       \node[invisibleboxnode, rotate=90]  (agent1)  at (0.5*\layersep cm, 0 cm) {asking agent};
       
    \end{tikzpicture}

==> GuessWhomodel_col.tex <==
        \def\layersep{3}
    \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep cm,        invisibleboxnode/.style={rounded corners=3pt, draw=none, fill=none, very thick, minimum width=25mm, minimum height=5mm, align=center},
]
        \tikzstyle{every pin edge}=[<-,shorten <=1pt]
        \tikzstyle{rnn}=[rectangle,minimum width=0.3*\layersep cm,minimum height=0.15*\layersep cm, fill=blue!15, draw=blue!50, thick,inner sep=1pt]{}
        \tikzstyle{elemwise}=[rectangle,minimum width=0.6*\layersep cm,minimum height=0.15*\layersep cm, fill=green!15, draw=green!50, thick,inner sep=1pt]{}
        \tikzstyle{qvals}=[rectangle,minimum width=0.6*\layersep cm,minimum height=0.1\layersep5* cm, fill=red!15, draw=red!50, thick,inner sep=1pt]{}
        \tikzstyle{variables}=[rectangle,minimum width=0.6*\layersep cm,minimum height=0.15*\layersep cm, thick,inner sep=1pt]{}        
        
            % \node[rnn, pin=left:$s_{0}$] (R1-1) at (\layersep cm, 0 cm) {};


            % \node[rnn,pin=left:$s_{1,0}$] (R2-1) at (\layersep cm, -\layersep*0.5 cm) {};
            
            % \node[rnn, pin={[pin edge={->}]right:$s_{3}$   ...}] (R1-3) at (\layersep*3 cm, 0 cm) {};
            % \node[rnn, pin={[pin edge={->}]right:$s_{1,3}$   ...}] (R2-3) at (\layersep*3 cm, -\layersep*0.5 cm) {};
        
        \foreach \name / \y in {1,...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[elemwise, pin=below:{\includegraphics[width=.05\linewidth]{guess_who/7.png}}
            {\includegraphics[width=.05\linewidth]{guess_who/22.png}}
            {\includegraphics[width=.05\linewidth]{guess_who/8.png}}
            {\includegraphics[width=.05\linewidth]{guess_who/5.png}}] (E1-\name) at (\layersep*\y cm, -\layersep*1*0.3 cm) {Elemwise add};
        
        \foreach \name / \y in {1,...,2}
            \node[qvals] (Q1-\name) at (\layersep*\y cm, \layersep*0.3cm) {DRU};
            
        \foreach \name / \y in {3,...,3}
            \node[qvals] (Q1-\name) at (\layersep*\y cm, \layersep*0.3cm) {$\epsilon$-greedy};
            
        \foreach \name / \y in {1,...,2}
            \node[variables] (V1-\name) at (\layersep*\y cm, \layersep*0.3cm + 0.25*\layersep cm) {$\hat{m}_{\y}^1$};
            
        \foreach \name / \y in {3,...,3}
            \node[variables] (V1-\name) at (\layersep*\y cm, \layersep*0.3cm + 0.25*\layersep cm) {$u^1$, \text{reward}};
  

        \foreach \name / \y in {1,...,3}
            \node[rnn] (R1-\name) at (\layersep*\y cm, 0 cm) {GRU};
            
        % \foreach \name / \y in {1,...,3}
        %     \node[rnn] (R2-\name) at (\layersep*\y cm, -\layersep*0.5 cm) {GRU};
            
        % \foreach \name / \y in {2, ...,3}
        %     \pgfmathsetmacro{\source}{int(\name-1)}
        %     \path (R2-\source) edge node[above, midway] {$h_{1,\source}$} (R2-\name);

        \foreach \name / \y in {2, ...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (R1-\source) edge node[above, midway] {$h^1_{\source}$} (R1-\name);


        % \foreach \name / \y in {1, ...,3}
        %     \path (R2-\name) edge node[right, midway] {$h_{1,\y}$} (R1-\name);
        
        \foreach \name / \y in {1, ...,2}
            \path (R1-\name) edge node[right, midway] {${m_\y^1}$} (Q1-\name);
            
        \foreach \name / \y in {3, ...,3}
            \path (R1-\name) edge node[right, midway] {${Q^1}$} (Q1-\name);
            
        \foreach \name / \y in {1, ...,3}
            \path (E1-\name) edge node[right, midway] {$z_{\y}^1$} (R1-\name); 
            
        \foreach \name / \y in {1, ...,3}
            \path (Q1-\name) edge (V1-\name);    
         
        \def\separate{1.3}
  
            
        %%%%%
        
        % \node[rnn, pin=left:$s_{0}$] (R21-1) at (\layersep cm + 0.5*\layersep cm,                    \separate*\layersep cm) {};
        
          \foreach \name / \y in {1,...,2}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[elemwise, pin=above:{\includegraphics[width=.05\textwidth]{guess_who/5.png}}] (E21-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm +\layersep*0.3cm) {Elemwise add};
        
        \foreach \name / \y in {1,...,2}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[qvals] (Q21-\name) at (\layersep * \y cm +  0.5 * \layersep cm, \separate * \layersep cm -\layersep * 0.3cm) {DRU};
            
         \foreach \name / \y in {1,...,2}           
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[variables] (V21-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm - \layersep*0.3cm - 0.25*\layersep cm) {${\hat{m}_{\y}^2}$(yes/no)};
            
        \foreach \name / \y in {1,...,2}
            \node[rnn] (R21-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm) {GRU};
            
        % \foreach \name / \y in {1,...,2}
        %     \node[rnn] (R22-\name) at (\layersep*\y cm + 0.5*\layersep cm, \separate*\layersep cm +\layersep*0.5 cm) {GRU};
            
        % \foreach \name / \y in {2, ...,2}
        %     \pgfmathsetmacro{\source}{int(\name-1)}
        %     \path (R22-\source) edge node[above, midway] {$h_{1,\source}$} (R22-\name);

        \foreach \name / \y in {2, ...,2}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (R21-\source) edge node[above, midway] {$h^2_{\source}$} (R21-\name);


        % \foreach \name / \y in {1, ...,2}
        %     \path (R22-\name) edge node[right, midway] {$h_{1,\y}$} (R21-\name);
        
        \foreach \name / \y in {1, ...,2}
            \path (R21-\name) edge node[right, midway] {${m_t^2}$} (Q21-\name);
            
        \foreach \name / \y in {1, ...,2}
            \path (E21-\name) edge node[right, midway] {$z_{\y}^2$} (R21-\name); 
        
        \foreach \name / \y in {1, ...,2}
            \path (Q21-\name) edge (V21-\name);
            
        \foreach \name / \y in {2, ...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (V21-\source) edge[thick,draw=black!85]  (E1-\name.160);
        \foreach \name / \y in {1, ...,2}
            \path (V1-\name) edge[thick,draw=black!85] (E21-\name.200);
            
         \node[draw,dotted,very thick,draw=black!60,fit=(R21-1) (R21-2) (Q21-1) (Q21-2) (E21-1) (E21-2)] (a2) {};
        
        \node[draw,dotted,very thick,draw=black!60,fit=(R1-1) (R1-3) (Q1-1) (Q1-3) (E1-1) (E1-3)] (a1) {};
         
        \node[invisibleboxnode,rotate=90]  (answering agent)  at (0.9*\layersep cm, \separate*\layersep cm) {answering agent};
        
       \node[invisibleboxnode, rotate=90]  (agent1)  at (0.4*\layersep cm, 0 cm) {asking agent};
      
       
    \end{tikzpicture}

==> model.tex <==
     \def\layersep{3.5}
    \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep cm,]
        \tikzstyle{every pin edge}=[<-,shorten <=1pt]
        \tikzstyle{rnn}=[rectangle,minimum width=1.5cm,minimum height=0.75cm, fill=blue!15, draw=blue!50, thick,inner sep=1pt]{}
        \tikzstyle{elemwise}=[rectangle,minimum width=3cm,minimum height=0.75cm, fill=green!15, draw=green!50, thick,inner sep=1pt]{}
        \tikzstyle{qvals}=[rectangle,minimum width=3cm,minimum height=0.75cm, fill=red!15, draw=red!50, thick,inner sep=1pt]{}
        
        \tikzstyle{mlp}=[rectangle,minimum width=1.5cm,minimum height=0.75cm, fill=orange!15, draw=orange!50, thick,inner sep=1pt]{}
        
            \node[rnn, pin=left:$h_{2,0}$] (R1-1) at (\layersep cm, 0 cm) {};
            \node[rnn,pin=left:$h_{1,0}$] (R2-1) at (\layersep cm, -\layersep*0.5 cm) {};
            
            \node[rnn, pin={[pin edge={->}]right:$h_{2,3}$   ...}] (R1-3) at (\layersep*3 cm, 0 cm) {};
            \node[rnn, pin={[pin edge={->}]right:$h_{1,3}$   ...}] (R2-3) at (\layersep*3 cm, -\layersep*0.5 cm) {};
        
        \foreach \name / \y in {1,...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[elemwise, pin=below:${(o^{a},\hat{m}_\source^{a'},u_\source^{a})}$] (E1-\name) at (\layersep*\y cm, -\layersep*2*0.5 cm) {Elemwise add};
        
        \foreach \name / \y in {1,...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[qvals, pin={[pin edge={->}]above:${u_{\y}^a, \hat{m}_{\y}^a}$}] (Q1-\name) at (\layersep*\y cm, \layersep cm) {$\epsilon$-greedy, DRU};
  
          \foreach \name / \y in {1,...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \node[mlp] (M1-\name) at (\layersep*\y cm, \layersep*0.5 cm) {MLP};
            
        \foreach \name / \y in {1,...,3}
            \node[rnn] (R1-\name) at (\layersep*\y cm, 0 cm) {GRU};
            
        \foreach \name / \y in {1,...,3}
            \node[rnn] (R2-\name) at (\layersep*\y cm, -\layersep*0.5 cm) {GRU};
            
        \foreach \name / \y in {2, ...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (R2-\source) edge node[above, midway] {$h_{1,\source}$} (R2-\name);

        \foreach \name / \y in {2, ...,3}
            \pgfmathsetmacro{\source}{int(\name-1)}
            \path (R1-\source) edge node[above, midway] {$h_{2,\source}$} (R1-\name);
            


        \foreach \name / \y in {1, ...,3}
            \path (R2-\name) edge node[right, midway] {$h_{1,\y}$} (R1-\name);
        
        \foreach \name / \y in {1, ...,3}
            \path (M1-\name) edge node[right, midway] {${Q_a, m_{\y}^a}$} (Q1-\name);
            
        \foreach \name / \y in {1, ...,3}
            \path (R1-\name) edge node[right, midway] {$h_{2,\y}$} (M1-\name);
            
        \foreach \name / \y in {1, ...,3}
            \path (E1-\name) edge node[right, midway] {$z_{\y}^a$} (R2-\name); 

    \end{tikzpicture}
